Underwater Image Super-Resolution using Deep Residual Multipliers

We present a deep residual network-based generative model for single image super-resolution (SISR) of underwater imagery for use by autonomous underwater robots. We also provide an adversarial training pipeline for learning SISR from paired data. In order to supervise the training, we formulate an objective function that evaluates the \textit{perceptual quality} of an image based on its global content, color, and local style information. Additionally, we present USR-248, a large-scale dataset of three sets of underwater images of 'high' (640x480) and 'low' (80x60, 160x120, and 320x240) spatial resolution. USR-248 contains paired instances for supervised training of 2x, 4x, or 8x SISR models. Furthermore, we validate the effectiveness of our proposed model through qualitative and quantitative experiments and compare the results with several state-of-the-art models' performances. We also analyze its practical feasibility for applications such as scene understanding and attention modeling in noisy visual conditions.

==> srctex/head.tex <==
\usepackage{graphicx} % for pdf, bitmapped graphics files
\usepackage{subcaption}
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed https://preview.overleaf.com/public/rsfmwkfvqdyp/images/8e680429ab22701a0e03ee380cd8785b240c35ed.jpeg
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
%\usepackage{svg}
%\usepackage{dsfont}
%\usepackage{hyperref}
\usepackage{csquotes}
\def\UrlBreaks{\do\/\do-}

\usepackage{array}
\usepackage{url} 
\usepackage{enumerate}
%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{multirow} % tables
%\usepackage{rotating} % for rotating texts
%\usepackage{subfigure}
\usepackage{float}
\usepackage{paralist}
\usepackage{amsfonts}
%\pagestyle{empty} % hiding page numbering
\sloppy % for tricky allignments
%\usepackage[justification=centering]{caption}
\usepackage{longtable}

%\usepackage{algorithmic}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Junaed's definition of a sidenote to look into
\newcommand{\marginlabel}[1]{\mbox{}\marginpar[\raggedleft\hspace{0pt}{#1}]{
		\raggedright\hspace{0pt}{#1}}}
\graphicspath{ {images/} }
\newcommand{\starnote}[1]{\marginlabel{$\bigstar$}\textbf{[#1]}}
% comment the previous line and uncomment the one below to remove all such notes in the output PDF
\newcommand{\nostarnote}[1]{}
\newcommand{\baad}[1]{} 
\usepackage[size=small]{caption}
%\usepackage{enumitem}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\etal}{\textit{et al.}} 
